Programmatic Reinforcement Learning: Navigating Gridworlds

The field of reinforcement learning (RL) is concerned with algorithms for learning optimal policies in unknown stochastic environments. Programmatic RL studies representations of policies as programs, meaning involving higher order constructs such as control loops. Despite attracting a lot of attention at the intersection of the machine learning and formal methods communities, very little is known on the theoretical front about programmatic RL: what are good classes of programmatic policies? How large are optimal programmatic policies? How can we learn them? The goal of this paper is to give first answers to these questions, initiating a theoretical study of programmatic RL. Considering a class of gridworld environments, we define a class of programmatic policies. Our main contributions are to place upper bounds on the size of optimal programmatic policies, and to construct an algorithm for synthesizing them. These theoretical findings are complemented by a prototype implementation of the algorithm.

==> definitions.tex <==
For simplicity, the environments we consider are discrete-time MDPs. The definitions we give here and the questions we ask can be naturally extended to more complicated environments, using for instance rewards functions or continuous time.

\begin{definition}[MDP]\label{def:mdp}
A markov decision process (MDP) is a tuple \((S, A, \delta, s_0, T)\) where \(S\) is a set of states, \(A\) is a finite set of actions, \(\delta : S \times A \to \mathscr{D}(S)\) is the transition function mapping a state and an action to a probability distribution over the state space, and \(s_0 \in S\) is the initial state.
\end{definition}
We refer to~\cite{mdpchapter} for the classical definitions (probabilistic space, policies, optimal policies). An MDP can be regarded as an environment in which an agent observes the current state of the game and picks an action to take following which the game updates the state using the transition function. Before presenting the PRISM syntax, let us consider the following example.

\begin{example}
The following codeblock defines an MDP in PRISM syntax\footnote{We deviate from PRISM syntax in cosmetic ways. PRISM supports specifying a wider range of stochastic models, for instance reward models for MDPs.}.
\begin{lstlisting}
x : [0..99] init 0;
y : [0..99] init 0;

[up] 	x < 10 && x + y >= 2 		-> 
	0.5 : y' = y + 1
	0.5 : y' = y + 1 && x' = x + 1;
[down] 	x < 10 && x + y >= 2 		-> 
	0.5 : y' = y - 1
	0.5 : y' = y - 1 && x' = x - 1;
[right] x < 10 && 3*x - y <= 20 	-> 
	1 : x' = x + 1;
\end{lstlisting}
The MDP specified here contains two state variables \texttt{x,y} which take integer values ranging from $0$ to $99$. The initial state is \texttt{(0,0)}. The MDP contains two regions which are specified by the predicates: \texttt{x < 10 \&\& x + y >= 2} and \texttt{x < 10 \&\& 3*x - y <= 20}. In the states where the first predicate is satisfied, two actions \texttt{up} and \texttt{down} are enabled. If in one of these states and the \texttt{up} action is picked by the agent, with \(0.5\) probability the next state is obtained by incrementing the \(y\)-coordinate by 1 and with \(0.5\) probability both \(x\) and \(y\) are incremented. 
\end{example}

We define now the idealised PRISM syntax. The state space is described by tuples of discrete variables. 
Each variable is specified by
\begin{lstlisting}
x : [n..m] init v;
\end{lstlisting}
where $n,m$ are integers and $v \in [n,m]$.
The rest of the program consists in a set of commands of the form
\begin{lstlisting}
[a] P(x) ->
  p1 : x' = delta(x,1)
  ...
  pn : x' = delta(x,n);
\end{lstlisting}
where $a$ is an action, $x,x'$ are states, $P$ is a predicate on states, $\delta : S \times [1,n] \to S$ is the update function computing the next state, and $\sum_i p_i = 1$.
The interpretation is as follows: from any state $x$ satisfying $P$, the action $a$ is available, and its effect is a random event: with probability $p_i$ we move to state $\delta(x,i)$.
In this idealised definition predicates and update functions are not restricted in any way (they should be at the very least computable).
We call \textit{environment programs} the class of environments defined by such programs, and happily identify programs and the environments they define.

The point of PRISM programs is that the use of predicates and update functions enable partitioning the state space into regions which have similar transitions, leading to very concise representations of large MDPs. For instance, the MDP given in the example above has $10.000$ states, but is given by $14$ lines of code.

Finally, we consider a specification, such as reaching a target state almost surely, then a policy is optimal if it satisfies the specification. We can now formulate the problem we study in this work in a very precise manner:

\begin{quotation}
Given a subclass of PRISM programs $\PEnv$, define a class of programmatic policies $\PPol$ such that
for each MDP definable by $\PEnv$, there exists an optimal policy given by some program $\sigma \in \PPol$.
\end{quotation}

